Efficient Kernel Object Management for Tiered Memory Systems with KLOC

Software-controlled heterogeneous memory systems have the potential to improve performance, efficiency, and cost tradeoffs in emerging systems. Delivering on this promise requires an efficient operating system (OS) mechanisms and policies for data management. Unfortunately, modern OSes do not support efficient tiering of data between heterogeneous memories. While this problem is known (and is being studied) for application-level data pages, the question of how best to tier OS kernel objects has largely been ignored. We show that careful kernel object management is vital to the performance of software-controlled tiered memory systems. We find that the state-of-the-art OS page management research leaves considerable performance on the table by overlooking how best to tier, migrate, and manage kernel objects like inodes, dentry caches, journal blocks, network socket buffers, etc., associated with the filesystem and networking stack. In response, we characterize hotness, reuse, and liveness properties of kernel objects to develop appropriate tiering/migration mechanisms and policies. We evaluate our proposal using a real-system emulation framework on large-scale workloads like RocksDB, Redis, Cassandra, and Spark and achieve 1.4X to 4X higher throughput compared to the prior art.

==> cmds.tex <==
\renewcommand{\ttdefault}{pxtt}

\newcommand{\URL}{\url}
\newcommand{\cc}[1]{\mbox{\smaller[0.5]\texttt{#1}}}

%\clubpenalty=10000
%\widowpenalty=10000

%\linespread{1.2}

%\fvset{fontsize=\scriptsize,xleftmargin=8pt,numbers=left,numbersep=5pt}

\input{code/fmt}
\newcommand{\figrule}{\hrule width \hsize height .33pt}
\newcommand{\coderule}{\vspace{-0.4em}\figrule}

\setlength{\abovedisplayskip}{0pt}
\setlength{\abovedisplayshortskip}{0pt}
\setlength{\belowdisplayskip}{0pt}
\setlength{\belowdisplayshortskip}{0pt}
\setlength{\jot}{0pt}

\def\Snospace~{\S{}}
\renewcommand*\sectionautorefname{\Snospace}
\def\sectionautorefname{\Snospace}
\def\subsectionautorefname{\Snospace}
\def\subsubsectionautorefname{\Snospace}
\def\chapterautorefname{\Snospace}
%\renewcommand{\figurename}{Fig.}
%\def\figureautorefname{\figurename}
\newcommand{\subfigureautorefname}{\figureautorefname}

%\numberwithin{equation}{section}
\newcommand{\yes}{Y}
\newcommand{\no}{}

% sema
\newcommand{\shl}{\ \cc{<}\cc{<}\ }
\newcommand{\shr}{\ \cc{>}\cc{>}\ }

\if 0
\renewcommand{\topfraction}{0.9}
\renewcommand{\dbltopfraction}{0.9}
\renewcommand{\bottomfraction}{0.8}
\renewcommand{\textfraction}{0.05}
\renewcommand{\floatpagefraction}{0.9}
\renewcommand{\dblfloatpagefraction}{0.9}
\setcounter{topnumber}{10}
\setcounter{bottomnumber}{10}
\setcounter{totalnumber}{10}
\setcounter{dbltopnumber}{10}
\fi

\newif\ifdraft\drafttrue
\newif\ifnotes\notestrue
\ifdraft\else\notesfalse\fi

% ref. http://en.wikibooks.org/wiki/LaTeX/Colors
\newcommand{\TK}[1]{\textcolor{LimeGreen}{TK: #1}}
\newcommand{\XXX}[1]{\textcolor{red}{XXX: #1}}
\newcommand{\TODO}[1]{\textcolor{Melon}{TODO: #1}}

% hide comments
% \renewcommand{\TK}[1]{\ignorespaces}
% \renewcommand{\XXX}[1]{\ignorespaces}
% \renewcommand{\TODO}[1]{\ignorespaces}

%% Ensure ligatures (e.g., ``fine official flag'') can be copy/pasted from PDF.
\input{glyphtounicode}
\pdfgentounicode=1

\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}

% include macros
\newcommand{\includepdf}[1]{
  \includegraphics[width=\columnwidth]{#1}
}
\newcommand{\includeplot}[1]{
  \resizebox{\columnwidth}{!}{\input{#1}}
}

% list
\newcommand{\squishlist}{
\begin{itemize}[noitemsep,nolistsep]
  \setlength{\itemsep}{-0pt}
}
\newcommand{\squishend}{
  \end{itemize}
}

%%
%% NOTE.
%%  to use circled number in caption, use
%%   (e.g., \protect\C{1})
%%
%\usepackage{tikz}
%\newcommand*\C[1]{%
%\begin{tikzpicture}[baseline=(C.base)]
%\node[draw,circle,inner sep=0.2pt](C) {#1};
%\end{tikzpicture}}

%\newcommand*\BC[1]{%
%\begin{tikzpicture}[baseline=(C.base)]
%\node[draw,circle,fill=black,inner sep=0.2pt](C) {\textcolor{white}{#1}};
%\end{tikzpicture}
%}


\usepackage{xstring}
\newcommand{\PP}[1]{
\vspace{2px}
\noindent{\bf \IfEndWith{#1}{.}{#1}{#1.}}
}

\newcommand{\V}{\checkmark}


==> rev.tex <==
\gdef\therev{0af9cc2}
\gdef\thedate{2016-05-07 21:07:04 -0400}


==> texfiles/designimpl.tex <==
\subsection{Implementation and Emulation}
We implement the DevFS prototype to understand the benefits and
implications of a file system inside a storage device. Due to the
current lack of programmable storage hardware, we implement DevFS as a
driver in the Linux 4 kernel and reserve DRAM at boot time to
emulate DevFS storage. We now describe our implementation of the DevFS
user-level library and device-level file system.

% with around 9K lines of code 

\noindent{\bf User-level library and interface. } 
DevFS utilizes command-based I/O, similar to modern storage hard-
ware such as NVMe~\cite{NVMeSpec, Xu:2015:NVMe}. The user library has
three primary responsibilities: to create a command buffer in host
memory, to convert the application’s POSIX interface into DevFS
commands and add them to the command buffer, and to ring a doorbell
for DevFS to process the request.
~\SK{When an application is initialized, the user-level library
creates a command buffer by making an ioctl call to the OS, which
allocates a DMA-able memory buffer, registers the allocated buffer,
and returns the virtual address of the buffer to the user-level library.}
~\SK{Currently, DevFS does not support sharing command
buffers across processes, and the buffer size is restricted by the Linux 
kernel allocation ({\em kmalloc()}) upper limit of 4~MB; 
these restrictions can be addressed by memory-mapping a larger region 
of shared memory in the kernel. The user-library adds I/O commands 
to the buffer and rings a
doorbell (emulated with an ioctl) with the address of the command
buffer from which DevFS can read I/O requests, perform permission
checks, and add them to a device-level I/O queue for processing.} For
simplicity, our current library implementation only supports
synchronous I/O operations: each command
has an I/O completion flag that will be set by DevFS, and the
user-library must wait until an I/O request completes. The 
user-library is implemented in about 2K lines of code.


\noindent{\bf DevFS file system. }
Because DevFS is a hardware-centric solution, DevFS uses
straightforward data structures and techniques that do not
substantially increase memory or CPU usage.~\SK{We extend PMFS with 
DevFS components and structures described earlier.} Regarding DevFS block 
management, each block in
DevFS is a memory page; pages for both metadata and data are allocated
from memory reserved for DevFS storage. The per-file memory journal
and I/O queue size are set to a default of 4~KB but are each
configurable during file system mount. The maximum number of
concurrently opened files or directories is limited by the number of
I/O queues and journals that can be created in DevFS memory. Finally,
DevFS does not yet support memory-mapped I/O. DevFS is implemented in
about 9K lines of code. 

\subsection{Discussion}
\label{impl}
\SK{Moving the file system inside a hardware device avoids OS 
interaction and allows applications to attain higher
performance. However, a device-level file system also introduces CPU
limitations and adds complexity in deploying new file system features.}

\noindent {\bf CPU limitations. } \SK{
The scalability and performance of DevFS is dependant on the
device-level CPU core count and their frequency. These device CPU
limitations can impact (a) applications (or a system with many
applications) that use several threads for frequent and non-dependant
I/O operations, (b) multi-threaded applications that are 
I/O read-intensive or metadata lookup-intensive, and finally, (c) CPU-intensive file system features
such as deduplication or compression. One possible approach to address
the CPU limitation is to identify file-system
operations and components that are CPU-intensive and move them to 
the user-level library in a manner that does not impact integrity, crash
consistency, and security. However, realizing this approach would
require extending DevFS to support a broader set of commands from 
the library in addition to application-level POSIX commands. Furthermore, we
believe that DevFS's direct-access benefits could motivate hardware
designers to increase CPU core count inside the storage device~\cite{BlueDBM},
thus alleviating the problem.}

\par \noindent {\bf Feature support. }
\SK{Moving the file system into storage complicates
the addition of new file system features, such as snapshots,
incremental backup, deduplication, or fixing bugs; additionally,
limited CPU and memory resources also add to the complexity. One
approach to solving this problem is by implementing features that can
be run in the background in software (OS or library), exposing the
storage device as a raw block device, and using host CPU and
memory. Another alternative is to support ``reverse computation'' by
offloading file system state and computation to the host.
Our future work will explore the feasibility of these approaches by
extending DevFS to support snapshots, deduplication, and software
RAID. Regarding bug fixes, changes to DevFS would require a firmware
upgrade, which is supported by most hardware vendors
today~\cite{firmupgrade}. Additionally, with increasing focus on
programmability of I/O hardware (e.g., NICs~\cite{Li:NIC, Moneta-D}) 
as dictated by new standards (e.g., NVMe), support for embedding
software into storage should become less challenging.}


==> texfiles/relwk.tex <==
\section{Related Work}
Significant prior work has focused on providing direct-access to
storage, moving computation to storage, or programmability of SSDs.

\noindent{\bf Direct-access storage. } 
Several hybrid user-level file system implementations, such as Intel's
SPDK~\cite{SPDK}, Light NVM~\cite{Bjorling:OpenChannel}, and Micron's
User Space NVME~\cite{micronvme} provide direct-access~\SK{to storage
by exposing them as a raw block device and exporting a userspace
device driver for block access.} Light NVM
goes one step further to enable I/O-intensive applications to
implement their own FTL. However, these approaches do not support
traditional file-system abstractions and instead
expose storage as a raw block device; they do not support
fundamental properties of a file system such as integrity,
concurrency, crash consistency, or security.

\noindent{\bf Computation inside storage. } 
Providing compute capability inside storage for performing batch tasks
have been explored for past four decades. Systems such as
CASSM~\cite{CASSM} and RARES~\cite{Lin:1976:RAP} have proposed adding
several processors to a disk for performing computation inside
storage. ActiveStorage~\cite{ActiveStore, Acharya:ActiveDisks} uses
one CPU inside a hard disk for performing database scans and search
operations, whereas
Smart-SSD~\cite{smart-ssd} is designed for query processing inside
SSDs. Architectures such as BlueDBM~\cite{BlueDBM} have shown the
benefits of scaling compute and DRAM inside flash memory for running
``big data'' applications. DevFS also uses device-level RAM and compute
capability; however, DevFS uses these resources for running a high-performance
file system that applications can use. 


\noindent{\bf Programmability. }
Willow~\cite{Seshadri:Willow} develops a system to
improve SSD programmability. Willow's I/O component is offloaded to an
SSD to bypass the OS and perform direct read and write operations.
However, without a centralized file system, Willow
also has the same general structural advantages and disadvantages of
hybrid user-level file systems.


==> texfiles/revisionplan.tex <==


1) Discussion subsection 

   a) Limited CPU count and CPU frequency (Review #80A, #80B, #80C, #80D, and #80E)
       Discussing the CPU-related limitations and its impact on applications that require high I/O parallelism

   b) Hardware-level file system limitations and work-around (Review #80B, Review #80D)

    -  Issues in terms of supporting existing features when a file-system
       is moved inside the hardware and possible ways to address them. The features include support
       for deduplication, RAID support copy-on-write snapshots.


 - Added Discussion subsection (4.7) after implementation to address the above concerns.


2) Security-related revision

    (Review #80A, #80C, #80D, and #80E)

    a)   Details of DevFS security mechanism and assumptions (e.g., unforgeable CPU ID).
    b)   How current design meets the bar of a POSIX-based file system?
    c)   Why context-switching does not impact security with our current design (Review #80E).


 - Changes to 4.5 in page 8


3) Design clarifications

    a)  Why reverse caching will not cause inconsistency issues because
         only inactive files are cached in the host (Review #80C, #80E)?

		
	Changes to 4.4 page 8, left-hand side paragraph.


    b)  Clarifying the details of command buffer  (Review #80C)
	 How command buffer allocated and is the size configurable? 
        Can the buffers be shared across processes? 

 
        Changes to 4.6 Implementation subsection


4. Other minor comments

Review #80C: Summary: "... DevFS can improve performance by more than 2x." As a summary, this is overselling the results. You have a best case of >2x for random 1k writes by a single process. All other cases are significantly less than that. It would be more useful to summarize with the range of results, and acknowdging the limitations. The summary in Section 5.3 has similar problems.

      
       Changes to 5.2 Summary



Section 4.1 says DevFS extends structures from PMFS. Later, Section 4.6 says you extend RamFS with the DevFS components and structures. Clarify.

    
       Clarified in 4.6  Page 9



Figure 2 caption and Section 4.1 say the filemap (or other per-file structures) are created during "file setup". Clarify if this means at file creation time, file open time, or if you are being deliberately vague because it could be either, and you later explore the tradeoffs of delaying the allocation of these structures until they are needed.


	Changes to 4.1 page 6 


Section 5.2, first paragraph: Filebench is not a workload. It could be described as a workload generator, but it supports a lot of different workload personalities.


       Changes to 5.2
        









